On Capacity Regions of Two-Receiver Broadcast Packet Erasure Channels with Feedback and Memory

The two-receiver broadcast packet erasure channel with feedback and memory is studied. Memory is modeled using a finite-state Markov chain representing a channel state. Outer and inner bounds on the capacity region are derived when the channel state is strictly causally known at the transmitter. The bounds are both formulated in terms of feasibility problems and they are matching in all but one of the constraints. The results are extended to feedback with larger delay. Numerical results show that the bounds are close in many examples and the gains offered through feedback can be quite large. The presented outer bound meets the inner bound recently derived in \cite{Kuo_Wang2014} and hence describes the capacity region.

==> figs/RateRegions_e1=0.6,e2=0.4,g1=0.3,g2=0.7.tex <==
% This file was created by matlab2tikz v0.4.4 running on MATLAB 8.3.
% Copyright (c) 2008--2013, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
%
% defining custom colors
\definecolor{mycolor1}{rgb}{0,1,1}%
%
\begin{tikzpicture}

\begin{axis}[%
width=11.0222222222222in,
height=8.59372222222222in,
scale only axis,
xmin=0,
xmax=0.5,
xlabel={$\text{R}_\text{1}$},
xmajorgrids,
ymin=0,
ymax=0.7,
ylabel={$\text{R}_\text{2}$},
ymajorgrids,
axis x line*=bottom,
axis y line*=left,
legend style={draw=black,fill=white,legend cell align=left}
]
\addplot [
color=red,
dashed,
line width=2.0pt
]
table[row sep=crcr]{
0 0.6\\
0.144075829383886 0.486255924170616\\
0.4 0\\
};
\addlegendentry{Memoryless BEC with FB};

\addplot [
color=red,
dotted,
line width=2.0pt
]
table[row sep=crcr]{
0 0.6\\
0.4 0\\
};
\addlegendentry{Memoryless BEC w/o FB};

\addplot [
color=red,
dash pattern=on 1pt off 3pt on 3pt off 3pt,
line width=2.0pt
]
table[row sep=crcr]{
0 0.6\\
0.16 0.6\\
0.4 0.36\\
0.4 0\\
};
\addlegendentry{Upper bound};

\addplot [
color=green,
solid,
line width=2.0pt,
mark=o,
mark options={solid}
]
table[row sep=crcr]{
0.00595498540036332 0.595498540036332\\
0.0785618827117829 0.54061393170235\\
0.133384291578115 0.49917287651377\\
0.166981234168073 0.473776459595414\\
0.169427933051308 0.47192696436989\\
0.171900649643586 0.470057801980179\\
0.174399373240486 0.468168980517908\\
0.176476698890697 0.465081489594173\\
0.178298851046507 0.461290165670959\\
0.180124656081216 0.457491241258887\\
0.185620968335914 0.44605514901256\\
0.200362192910603 0.415383310105322\\
0.277333899042903 0.255229466783594\\
0.374773597508212 0.0524881870917156\\
0.392868268095032 0.0148388847215831\\
0.396743370472421 0.00677601889479151\\
0.39778400223793 0.00461079240958768\\
0.398086751102223 0.00398086751102223\\
};
\addlegendentry{Algorithm B};

\addplot [
color=blue,
dashed,
line width=2.0pt,
mark=+,
mark options={solid}
]
table[row sep=crcr]{
0.00595436574357171 0.595436574357171\\
0.00629065087301608 0.59517884544882\\
0.0194215356055592 0.585115335969878\\
0.0589149864797912 0.554847556964554\\
0.13512525219515 0.496440012687017\\
0.164088666270139 0.474242453419452\\
0.166495381197647 0.47239794720533\\
0.168426947154951 0.469138804076974\\
0.186638201310049 0.432245020926906\\
0.370828137733954 0.0590986403990124\\
0.3919852341098 0.0162369396546382\\
0.395680625806126 0.00875052610301388\\
0.397459588371972 0.00514656458682978\\
0.397885494110922 0.00428373142655511\\
0.397998827669093 0.00405413143947138\\
0.398035245939133 0.00398035245939133\\
};
\addlegendentry{Algorithm C};

\addplot [
color=black,
dashed,
line width=2.0pt,
mark=square,
mark options={solid}
]
table[row sep=crcr]{
0.00594237695078031 0.594237695078031\\
0.00937394125721534 0.590910117568761\\
0.0127578181185331 0.587628782430514\\
0.127332755703847 0.476525812650815\\
0.131106506186891 0.472866418243015\\
0.132870967925471 0.470466056489469\\
0.134513830830454 0.46757265614935\\
0.139501392464867 0.458788592375308\\
0.20952511943701 0.335463222484072\\
0.352941602717827 0.0828789683477082\\
0.393482986596523 0.0114777250986615\\
0.397080584584786 0.0051416569999292\\
0.397236760176505 0.00486660148018471\\
0.397741636470886 0.00397741636470886\\
};
\addlegendentry{Algorithm D};

\addplot [
color=blue,
solid,
line width=2.0pt,
mark=+,
mark options={solid}
]
table[row sep=crcr]{
3.4496197043767e-17 0.6\\
0.167014623405722 0.472\\
0.231430452035778 0.399747230997454\\
0.32968126878715 0.184791226432981\\
0.4 2.36592492072044e-17\\
};
\addlegendentry{Algorithm C weighted};

\addplot [
color=black,
solid,
line width=2.0pt,
mark=square,
mark options={solid}
]
table[row sep=crcr]{
0 0.6\\
0.132 0.472\\
0.22 0.36\\
0.328 0.168\\
0.4 0\\
};
\addlegendentry{Algorithm D weighted};

\addplot [
color=mycolor1,
solid,
line width=2.0pt,
mark=x,
mark options={solid}
]
table[row sep=crcr]{
2.58497232509185e-10 0.599999999736902\\
2.72033729867497e-10 0.599999999691739\\
0.189599999192191 0.47200000038028\\
0.199830675737066 0.463720840010873\\
0.199830681174372 0.463720834732373\\
0.199830684604842 0.463720831085207\\
0.220000001003401 0.431999997231638\\
0.32799999900388 0.189600001315286\\
0.399999998930987 1.31500233841805e-09\\
0.399999999844793 2.75542187748282e-10\\
};
\addlegendentry{Cap};

\addplot [
color=blue,
solid,
line width=1.0pt,
mark=square,
mark options={solid},
forget plot
]
table[row sep=crcr]{
0 0\\
0.072 0\\
0.088 0\\
0.108 0\\
0.132 0\\
0.16 0\\
0.18 0\\
0.196 0\\
0.204 0\\
0.22 0\\
0.24 0\\
0.268 0\\
0.292 0\\
0.312 0\\
0.328 0\\
0.4 0\\
0.340362231345086 0.157046124124608\\
0.267064246191321 0.321559379691946\\
0.213642813195244 0.405576724313048\\
0.162561486983413 0.478948083780951\\
0.150199255638328 0.489901959656344\\
0.115620688634404 0.517884615035241\\
0.0809186737881689 0.545371359467903\\
0 0.6\\
0 0.488\\
0 0.472\\
0 0.432\\
0 0.408\\
0 0.36\\
0 0.32\\
0 0.304\\
0 0.296\\
0 0.28\\
0 0.24\\
0 0.192\\
0 0.168\\
0 0.128\\
0 0.112\\
0 0\\
};
\end{axis}
\end{tikzpicture}%

==> figs/RateRegions_e1=0.6,e2=0.5,g1=0.1,g2=0.1.tex <==
% This file was created by matlab2tikz v0.4.4 running on MATLAB 8.3.
% Copyright (c) 2008--2013, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
%
% defining custom colors
\definecolor{mycolor1}{rgb}{0,1,1}%
%
\begin{tikzpicture}[scale=0.3]

\begin{axis}[%
width=4.82222222222222in,
height=3.80333333333333in,
scale only axis,
xmin=0,
xmax=0.5,
xlabel={$R_1$},
xmajorgrids,
ymin=0,
ymax=0.6,
ylabel={$R_2$},
ymajorgrids,
axis x line*=bottom,
axis y line*=left,
legend style={draw=black,fill=white,legend cell align=left}
]
\addplot [
color=red,
dashed,
line width=2.0pt
]
table[row sep=crcr]{
0 0.5\\
0.193103448275862 0.362068965517241\\
0.4 0\\
};
\addlegendentry{$\mc C_{\text{fb}}$: Memoryless BPEC with FB};

\addplot [
color=red,
dotted,
line width=2.0pt
]
table[row sep=crcr]{
0 0.5\\
0.4 0\\
};
\addlegendentry{$\mc C$: Memoryless BPEC w/o FB};

\addplot [
color=red,
dash pattern=on 1pt off 3pt on 3pt off 3pt,
line width=2.0pt
]
table[row sep=crcr]{
0 0.5\\
0.2 0.5\\
0.4 0.3\\
0.4 0\\
};
\addlegendentry{Geenie-aided outer bound};




\addplot [
color=mycolor1,
solid,
line width=2.0pt,
mark=x,
mark options={solid}
]
table[row sep=crcr]{
3.44136977755824e-09 0.499999999526105\\
0.17299999920745 0.480000000014933\\
0.172999999338219 0.479999999987996\\
0.215561610400847 0.457599152249845\\
0.341503094202182 0.32714412037357\\
0.369999999876739 0.272999999992967\\
0.370000000000244 0.272999999542705\\
0.399999999370706 5.22349492899921e-09\\
};
\addlegendentry{$\mc C_{\text{fb}}^{\text{mem}}$: Capacity region };

\end{axis}
\end{tikzpicture}%
